TokEval: A Tokenizer Evaluation Suite

Language model tokenizers are typically selected with minimal evaluation, despite the fact that their design choices directly impact model capabilities. This can be partly attributed to a limited understanding of which tokenizer properties affect which aspects of downstream performance. We introduce TokEval, a framework of tokenizer evaluation metrics that goes beyond standard measures like fertility and compression rate to capture linguistically and structurally meaningful properties, e.g., UTF-8 character boundary integrity and digit place-value boundary alignment for mathematics. To validate whether these metrics are predictive of downstream model performance, we conduct controlled language model pretraining experiments, varying solely the tokenizers' training data mixture, pretokenization strategy, and training algorithm. We evaluate the resulting models on bits-per-byte (a tokenizer-agnostic version of perplexity) and several benchmarks, spanning linguistic understanding, mathematical reasoning, and code generation. Our experiments suggest that different intrinsic properties have different impacts on model abilities: information-theoretic metrics predict language modeling abilities (Spearman rho up to 0.80), while structure-sensitive metrics, such as those measuring digit and line-break handling, correlate with task accuracy. We hope TokEval enables more principled tokenizer evaluation, replacing pretraining sweeps with intrinsic measurement wherever the two agree.

==> tables_camera_ready/aggregate-correlations-body.tex <==
% Body of tab:aggregate-correlations in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% n=29 for most columns (n=19 for ['code_bpb_mc20b', 'mbpp_mc20b']) tokenizers -- keep the caption's stated n in sync with this (hand-maintained, not auto-inserted).
% BH-FDR family for the stars below: 98 tests (14 intrinsic metrics x 7 printed downstream columns) -- keep the caption's stated family size in sync.
\small
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Intrinsic Metric}} & \multirow{2}{*}{\textbf{Val BPB}} & \multicolumn{2}{c}{\textbf{FLORES}} & \multicolumn{2}{c}{\textbf{Math+code}} & \multirow{2}{*}{\textbf{BLiMP}} & \multirow{2}{*}{\textbf{MultiBLiMP}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 &  & \textbf{trained} & \textbf{all} & \textbf{Code BPB} & \textbf{MBPP} &  &  \\
\midrule
R\'enyi eff.\ ($\alpha$=2) & $\textbf{-0.57}^{*}$ & $\textbf{-0.80}^{***}$ & $-0.39$ & $-0.49$ & $0.21$ & $-0.32$ & $0.37$ \\
Digit boundary F1 & $-0.42$ & $-0.41$ & $\textbf{-0.67}^{**}$ & $\textbf{-0.62}^{*}$ & $0.21$ & $\textbf{-0.51}^{*}$ & $0.32$ \\
Ident.\ fragmentation & $\textbf{0.53}^{*}$ & $\textbf{0.57}^{*}$ & $0.36$ & $0.41$ & $-0.21$ & $0.37$ & $-0.45$ \\
Operator isolation (math) & $\textbf{0.54}^{*}$ & $0.38$ & $\textbf{0.55}^{*}$ & $0.39$ & $0.27$ & $0.32$ & $-0.25$ \\
UTF-8 boundary crossing & $0.29$ & $\textbf{0.47}^{*}$ & $-0.21$ & $0.45$ & $-0.42$ & $0.27$ & $-0.41$ \\
Trigram entropy & $-0.44$ & $\textbf{-0.66}^{**}$ & $0.12$ & $-0.45$ & $0.10$ & $-0.05$ & $\textbf{0.48}^{*}$ \\
UTF-8 char split & $0.36$ & $\textbf{0.54}^{*}$ & $-0.34$ & $0.24$ & $-0.24$ & $0.09$ & $-0.40$ \\
Compression rate & $-0.32$ & $\textbf{-0.51}^{*}$ & $0.24$ & $-0.12$ & $0.26$ & $-0.14$ & $0.28$ \\
Bigram entropy & $-0.35$ & $\textbf{-0.52}^{*}$ & $0.00$ & $-0.18$ & $0.04$ & $-0.27$ & $0.35$ \\
Vocab utilization & $0.14$ & $-0.07$ & $\textbf{0.61}^{**}$ & $0.56$ & $0.07$ & $0.21$ & $0.02$ \\
AST alignment & $0.31$ & $0.01$ & $0.36$ & $0.16$ & $\textbf{0.61}^{*}$ & $0.10$ & $-0.05$ \\
Fertility & $0.04$ & $0.22$ & $\textbf{-0.57}^{*}$ & $-0.39$ & $0.09$ & $-0.18$ & $-0.08$ \\
Unigram entropy & $-0.27$ & $\textbf{-0.49}^{*}$ & $0.07$ & $-0.02$ & $0.25$ & $-0.22$ & $0.25$ \\
Gini coefficient & $-0.03$ & $0.18$ & $\textbf{-0.58}^{*}$ & $-0.37$ & $0.08$ & $-0.17$ & $-0.03$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/aggregate-correlations-fineweb-body.tex <==
% Body of tab:aggregate-correlations-fineweb in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% n=29 for most columns (n=19 for ['code_bpb_mc20b', 'mbpp_mc20b']) tokenizers -- keep the caption's stated n in sync with this (hand-maintained, not auto-inserted).
% BH-FDR family for the stars below: 98 tests (14 intrinsic metrics x 7 printed downstream columns) -- keep the caption's stated family size in sync.
\small
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Intrinsic Metric}} & \multirow{2}{*}{\textbf{Val BPB}} & \multicolumn{2}{c}{\textbf{FLORES}} & \multicolumn{2}{c}{\textbf{Math+code}} & \multirow{2}{*}{\textbf{BLiMP}} & \multirow{2}{*}{\textbf{MultiBLiMP}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 &  & \textbf{trained} & \textbf{all} & \textbf{Code BPB} & \textbf{MBPP} &  &  \\
\midrule
Digit boundary F1 & $-0.42$ & $-0.41$ & $\textbf{-0.67}^{**}$ & $\textbf{-0.62}^{*}$ & $0.21$ & $\textbf{-0.51}^{*}$ & $0.32$ \\
Ident.\ fragmentation & $\textbf{0.53}^{*}$ & $\textbf{0.57}^{*}$ & $0.36$ & $0.41$ & $-0.21$ & $0.37$ & $-0.45$ \\
R\'enyi eff.\ ($\alpha$=2) & $\textbf{-0.53}^{*}$ & $\textbf{-0.72}^{***}$ & $-0.42$ & $-0.49$ & $0.12$ & $-0.25$ & $0.32$ \\
Operator isolation (math) & $\textbf{0.54}^{*}$ & $0.38$ & $\textbf{0.55}^{*}$ & $0.39$ & $0.27$ & $0.32$ & $-0.25$ \\
Gini coefficient & $0.33$ & $\textbf{0.62}^{**}$ & $0.38$ & $\textbf{0.60}^{*}$ & $-0.10$ & $0.24$ & $-0.36$ \\
UTF-8 char split & $0.38$ & $\textbf{0.56}^{*}$ & $-0.33$ & $0.25$ & $-0.26$ & $0.09$ & $-0.43$ \\
Vocab utilization & $0.26$ & $0.07$ & $\textbf{0.70}^{**}$ & $0.54$ & $0.05$ & $0.32$ & $-0.17$ \\
Trigram entropy & $-0.37$ & $\textbf{-0.54}^{*}$ & $0.12$ & $-0.28$ & $0.08$ & $-0.14$ & $0.33$ \\
UTF-8 boundary crossing & $0.18$ & $0.34$ & $-0.33$ & $0.20$ & $-0.27$ & $0.18$ & $-0.33$ \\
Fertility & $0.27$ & $0.41$ & $-0.37$ & $0.16$ & $0.23$ & $-0.04$ & $-0.28$ \\
Compression rate & $-0.32$ & $-0.47$ & $0.24$ & $-0.19$ & $-0.03$ & $-0.17$ & $0.28$ \\
Bigram entropy & $-0.35$ & $\textbf{-0.53}^{*}$ & $0.00$ & $-0.21$ & $-0.02$ & $-0.23$ & $0.30$ \\
AST alignment & $0.31$ & $0.01$ & $0.36$ & $0.16$ & $\textbf{0.61}^{*}$ & $0.10$ & $-0.05$ \\
Unigram entropy & $-0.34$ & $\textbf{-0.51}^{*}$ & $0.04$ & $-0.12$ & $0.04$ & $-0.22$ & $0.26$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/axes2-grid-body.tex <==
% Body of tab:axes2-grid in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% Reformats results/correlations/axes2_codegrad_v2.json (produced by scripts/analyze_axes2_codegrad.py) -- this script does not recompute these values.
% Generated by scripts/generate_ablation_std1b_tables.py. DO NOT EDIT BY HAND.
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Regex} & \textbf{0\% code} & \textbf{5\% code} & \textbf{30\% code} & \textbf{50\% code} \\
\midrule
fusing (\texttt{gpt4o}) & $0.2320$ & $0.0500$ & $0.1780$ & $0.0880$ \\
non-fusing (\texttt{gpt4onl}) & $0.2480$ & $0.2060$ & $0.2240$ & $0.2120$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/cross-regime-code-bpb-body.tex <==
% Body of tab:cross-regime-code-bpb in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% Generated by scripts/analyze_cross_regime_code_bpb.py. DO NOT EDIT BY HAND.
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Tokenizer} & \textbf{\crnew{Natural-language} BPB} & \textbf{\crnew{Natural-language} rank} & \textbf{Math+code BPB} & \textbf{Math+code rank} \\
\midrule
MinGram SCRIPT-enc & $0.5125$ & $1.0$ & $0.3793$ & $9.0$ \\
BPE SCRIPT-enc GPT-4o & $0.5186$ & $2.0$ & $0.3781$ & $6.0$ \\
BPE Claude (bal.) & $0.5203$ & $3.0$ & $0.3861$ & $18.0$ \\
BPE GPT-4o (bal.)$^{*}$ & $0.5206$ & $4.0$ & $0.3773$ & $5.0$ \\
BPE Claude NFC & $0.5206$ & $5.0$ & $0.3845$ & $17.0$ \\
BPE GPT-4o NFC & $0.5207$ & $6.0$ & $0.3786$ & $8.0$ \\
BPE RightAlign (bal.) & $0.5223$ & $7.0$ & $0.3798$ & $10.0$ \\
BPE RightAlign NFC & $0.5225$ & $8.0$ & $0.3809$ & $13.0$ \\
BPE NFC clean (bal.) & $0.5226$ & $9.0$ & $0.3815$ & $14.0$ \\
BPE NFC clean plus3 (bal.) & $0.5232$ & $10.0$ & $0.3834$ & $16.0$ \\
BPE NFC clean plus2 (bal.) & $0.5249$ & $11.0$ & $0.3785$ & $7.0$ \\
SuperBPE GPT-4o (bal.) & $0.5249$ & $12.0$ & $0.3834$ & $15.0$ \\
SuperBPE clean C2 (bal.) & $0.5259$ & $13.0$ & $0.3906$ & $21.0$ \\
BPE Whitespace (bal.)$^\dagger$ & $0.5269$ & $14.0$ & $0.3742$ & $4.0$ \\
BPE Punct (bal.) & $0.5302$ & $15.0$ & $0.3801$ & $11.0$ \\
SuperBPE clean C3 (bal.) & $0.5306$ & $16.0$ & $0.3896$ & $20.0$ \\
PA-BPE NFC GPT-4o & $0.5335$ & $17.0$ & $0.3878$ & $19.0$ \\
BPE Claude (eng.) & $0.5426$ & $18.0$ & $0.3652$ & $1.0$ \\
BPE GPT-4o (code) & $0.5447$ & $19.0$ & $0.3805$ & $12.0$ \\
BPE Punct (eng.) & $0.5551$ & $20.0$ & $0.3724$ & $3.0$ \\
Unigram RightAlign & $0.5566$ & $21.0$ & $0.3989$ & $22.0$ \\
BPE GPT-4o (eng.) & $0.5567$ & $22.0$ & $0.3709$ & $2.0$ \\
BPE GPT-4o (eng., full-byte) & $0.5568$ & $23.0$ & $0.3991$ & $23.0$ \\
Unigram GPT-4o & $0.5569$ & $24.0$ & $0.3993$ & $24.0$ \\
Unigram Claude & $0.5578$ & $25.0$ & $0.4032$ & $25.0$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/cross-scale-ranking-body.tex <==
% Body of tab:cross-scale-ranking in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% Generated by scripts/analyze_cross_scale_ranking.py. DO NOT EDIT BY HAND.
\begin{tabular}{lcccc}
\toprule
 & \textbf{d8 (tiny)} & \textbf{d12 (small)} & \textbf{d16 (pilot)} & \textbf{d24 (full)} \\
\midrule
\textbf{d8 (tiny)} & $1.000$ & $0.882$ & $0.882$ & $0.765$ \\
\textbf{d12 (small)} & $0.882$ & $1.000$ & $0.922$ & $0.725$ \\
\textbf{d16 (pilot)} & $0.882$ & $0.922$ & $1.000$ & $0.752$ \\
\textbf{d24 (full)} & $0.765$ & $0.725$ & $0.752$ & $1.000$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/data-composition-body.tex <==
% Body of tab:data-composition in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_data_composition_table.py from the mixture manifest.
\small
\begin{tabular}{llrr}
\toprule
\textbf{Domain} & \textbf{Source} & \textbf{Bytes} & \textbf{\%} \\
\midrule
English web           & FineWeb-Edu    & 9.2\,GB & 36.9 \\
Multilingual (30 langs)& FineWeb2       & 8.3\,GB & 33.4 \\
Math                  & FineMath-4plus & 4.0\,GB & 16.1 \\
Code (Python)         & StarCoderData  & 2.5\,GB & 10.0 \\
Code (JavaScript)     & StarCoderData  & 0.9\,GB &  3.6 \\
\midrule
\textbf{Total}        &                & \textbf{25.0\,GB} & 100.0 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/heldout-reference-body.tex <==
% Generated by scripts/analyze_heldout_reference_prediction.py --latex. DO NOT EDIT.
% prov: results/correlations/heldout_reference_prediction.json#targets.*
% source artifact generated at 2026-08-17T16:45:22+00:00 (commit caf402b28f38)
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}p{2.3cm}l p{3.5cm} c c r r@{}}
\toprule
 & & & & & \multicolumn{2}{c}{Standardized error} \\
\cmidrule(lr){6-7}
Target & Fit & Predictors & $R^2$ & CV-RMSE & \shortstack[r]{Mistral-\\Nemo} & LLaMA-3 \\
\midrule
Val BPB ($n{=}39$) & univ. & tokens per identifier & 0.53 & 0.0061 & $+0.48$ & $+1.43$ \\
 & multiv. & fertility, Gini coefficient, tokens per identifier & 0.68 & 0.0054 & $+0.35$ & $+1.84^{\dagger}$ \\
\addlinespace
FLORES (trained) BPB ($n{=}39$) & univ. & identifier fragmentation & 0.59 & 0.0091 & $+0.36$ & $+2.10^{\dagger}$ \\
 & multiv. & fertility, identifier fragmentation, indentation consistency & 0.81 & 0.0062 & $+0.41$ & $+2.18^{\dagger}$ \\
\addlinespace
Code BPB (math+code) ($n{=}20$) & univ. & Gini coefficient (FineWeb) & 0.48 & 0.0074 & $-0.40$ & $-2.01^{\dagger}$ \\
 & multiv. & vocabulary utilization (FineWeb), trigram entropy, operator isolation (code corpus) & 0.68 & 0.0070 & $-0.05$ & $-0.90$ \\
\addlinespace
MBPP pass@1 (math+code) ($n{=}20$) & univ. & AST boundary alignment & 0.26 & 0.0793 & $-1.15$ & $-0.03$ \\
 & multiv. & token length, unigram entropy, AST boundary alignment & 0.50 & 0.0739 & $-1.78^{\dagger}$ & $+1.77^{\dagger}$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/intrinsic-fineweb-body.tex <==
% Body of tab:intrinsic-fineweb in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_intrinsic_tables.py --dataset fineweb --panel std1b (roster: generate_latex_tables.STD1B_MAIN_ROSTER when --panel std1b).
\small
\adjustbox{max width=\textwidth}{%
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Tokenizer} & \textbf{Fertility} $\downarrow$ & \textbf{Compression} $\uparrow$ & \textbf{Gini} $\downarrow$ & \textbf{Vocab CoV} $\downarrow$ & \textbf{$\bar H_2$} $\uparrow$ & \textbf{Bigram $\eta$} $\uparrow$ & \textbf{Char Split} $\downarrow$ \\
\midrule
Mistral-Nemo$^\dagger$ & 4.82 {\scriptsize $\pm$13.94} & 4.2326 & 0.128 & 0.396 & 0.572 & 0.787 & 0.010 \\
LLaMA-3$^\dagger$ & 5.15 {\scriptsize $\pm$12.40} & 3.5226 & 0.161 & 0.388 & 0.542 & 0.734 & 0.105 \\
\midrule
BPE Punct (bal.) & 4.73 {\scriptsize $\pm$11.64} & 3.9624 & 0.111 & 0.417 & 0.533 & 0.760 & 0.028 \\
BPE Punct (eng.) & 8.90 {\scriptsize $\pm$26.00} & 2.4434 & 0.135 & 0.534 & 0.519 & 0.669 & 0.226 \\
BPE GPT-4o (bal.) & 4.36 {\scriptsize $\pm$11.29} & 4.2847 & 0.132 & 0.407 & 0.578 & 0.801 & 0.033 \\
BPE GPT-4o NFC & 4.36 {\scriptsize $\pm$11.29} & 4.2847 & 0.132 & 0.407 & 0.578 & 0.801 & 0.033 \\
BPE GPT-4o (eng.) & 8.95 {\scriptsize $\pm$26.20} & 2.4458 & 0.140 & 0.537 & 0.523 & 0.678 & 0.259 \\
BPE GPT-4o (eng., full-byte) & 8.95 {\scriptsize $\pm$26.21} & 2.4455 & 0.140 & 0.537 & 0.523 & 0.678 & 0.259 \\
BPE GPT-4o (code) & 6.93 {\scriptsize $\pm$16.48} & 2.6289 & 0.103 & 0.501 & 0.538 & 0.681 & 0.200 \\
BPE Claude (bal.) & 4.42 {\scriptsize $\pm$11.55} & 4.2538 & 0.132 & 0.414 & 0.544 & 0.791 & 0.032 \\
BPE Claude NFC & 4.42 {\scriptsize $\pm$11.55} & 4.2538 & 0.132 & 0.414 & 0.544 & 0.791 & 0.032 \\
BPE Claude (eng.) & 8.89 {\scriptsize $\pm$26.05} & 2.4553 & 0.135 & 0.540 & 0.522 & 0.677 & 0.246 \\
BPE RightAlign (bal.) & 4.36 {\scriptsize $\pm$11.29} & 4.2847 & 0.132 & 0.405 & 0.578 & 0.801 & 0.033 \\
BPE RightAlign NFC & 4.36 {\scriptsize $\pm$11.29} & 4.2847 & 0.132 & 0.405 & 0.578 & 0.801 & 0.033 \\
Unigram GPT-4o & 4.40 {\scriptsize $\pm$9.11} & 3.5065 & 0.175 & 0.365 & 0.326 & 0.684 & 0.044 \\
Unigram Claude & 4.51 {\scriptsize $\pm$9.64} & 3.4771 & 0.173 & 0.365 & 0.335 & 0.679 & 0.049 \\
Unigram RightAlign & 4.40 {\scriptsize $\pm$9.11} & 3.5064 & 0.175 & 0.365 & 0.326 & 0.684 & 0.044 \\
SuperBPE GPT-4o (bal.) & 4.41 {\scriptsize $\pm$11.46} & 4.2975 & 0.128 & 0.451 & 0.665 & 0.818 & 0.038 \\
PA-BPE NFC GPT-4o & 4.20 {\scriptsize $\pm$12.48} & 4.8100 & 0.146 & 0.259 & 0.562 & 0.826 & 0.017 \\
Unigram GPT-4o (highmid) & 4.93 {\scriptsize $\pm$9.03} & 3.0457 & 0.179 & 0.400 & 0.338 & 0.660 & 0.154 \\
Unigram GPT-4o (highres) & 5.89 {\scriptsize $\pm$11.19} & 2.6422 & 0.163 & 0.516 & 0.334 & 0.638 & 0.200 \\
MinGram SCRIPT-enc & 4.33 {\scriptsize $\pm$11.42} & 4.3649 & 0.130 & 0.403 & 0.526 & 0.792 & 0.000 \\
MinGram SCRIPT-enc (nl-split) & 4.33 {\scriptsize $\pm$11.42} & 4.3654 & 0.130 & 0.403 & 0.526 & 0.792 & 0.000 \\
BPE SCRIPT-enc GPT-4o & 4.35 {\scriptsize $\pm$11.28} & 4.3009 & 0.132 & 0.402 & 0.572 & 0.801 & 0.000 \\
BPE GPT-2 (bal.) & 4.70 {\scriptsize $\pm$11.62} & 4.0035 & 0.112 & 0.411 & 0.546 & 0.765 & 0.029 \\
BPE GPT-4o (all-eq.) & 4.18 {\scriptsize $\pm$12.10} & 4.7119 & 0.140 & 0.359 & 0.566 & 0.823 & 0.017 \\
BPE Claude (all-eq.) & 4.24 {\scriptsize $\pm$12.28} & 4.6684 & 0.142 & 0.360 & 0.531 & 0.811 & 0.016 \\
BPE Punct (all-eq.) & 4.62 {\scriptsize $\pm$12.21} & 4.2193 & 0.091 & 0.383 & 0.525 & 0.765 & 0.015 \\
BPE GPT-4o NFC (all-eq.) & 4.18 {\scriptsize $\pm$12.10} & 4.7119 & 0.140 & 0.359 & 0.566 & 0.823 & 0.017 \\
BPE GPT-4o (all-eq., no-rep.) & 4.18 {\scriptsize $\pm$12.10} & 4.7119 & 0.140 & 0.359 & 0.566 & 0.823 & 0.017 \\
BPE GPT-4o (bal., mf50) & 4.36 {\scriptsize $\pm$11.29} & 4.2847 & 0.132 & 0.407 & 0.578 & 0.801 & 0.033 \\
BPE NFC clean (bal.) & 4.42 {\scriptsize $\pm$11.18} & 4.2056 & 0.113 & 0.413 & 0.541 & 0.783 & 0.033 \\
BPE NFC clean plus2 (bal.) & 4.47 {\scriptsize $\pm$11.64} & 4.2161 & 0.132 & 0.425 & 0.541 & 0.783 & 0.031 \\
BPE NFC clean plus3 (bal.) & 4.47 {\scriptsize $\pm$11.65} & 4.2127 & 0.132 & 0.425 & 0.541 & 0.783 & 0.031 \\
SuperBPE PA-BPE GPT-4o & 4.16 {\scriptsize $\pm$12.35} & 4.9042 & 0.145 & 0.330 & 0.642 & 0.846 & 0.019 \\
SuperBPE PA-BPE GPT-4o t64k & 4.14 {\scriptsize $\pm$11.92} & 4.8166 & 0.143 & 0.383 & 0.657 & 0.844 & 0.020 \\
SuperBPE clean C2 (bal.) & 4.31 {\scriptsize $\pm$12.51} & 4.6590 & 0.145 & 0.373 & 0.529 & 0.809 & 0.018 \\
SuperBPE clean C3 (bal.) & 4.19 {\scriptsize $\pm$12.27} & 4.8310 & 0.144 & 0.345 & 0.592 & 0.835 & 0.019 \\
SuperBPE Punct t64k & 4.46 {\scriptsize $\pm$11.38} & 4.2271 & 0.120 & 0.443 & 0.626 & 0.810 & 0.034 \\
PA-BPE NFC GPT-4o HW & 4.12 {\scriptsize $\pm$12.01} & 4.8303 & 0.140 & 0.287 & 0.563 & 0.828 & 0.016 \\
PA-BPE NFC clean & 4.38 {\scriptsize $\pm$12.98} & 4.6207 & 0.146 & 0.273 & 0.527 & 0.801 & 0.018 \\
Unigram GPT-4o tuned & 4.40 {\scriptsize $\pm$9.21} & 3.5078 & 0.171 & 0.374 & 0.329 & 0.690 & 0.045 \\
BPE GPT-4o (highres) & 6.49 {\scriptsize $\pm$14.16} & 2.7379 & 0.183 & 0.483 & 0.505 & 0.677 & 0.227 \\
BPE GPT-4o (highmid) & 5.07 {\scriptsize $\pm$11.34} & 3.4759 & 0.207 & 0.417 & 0.504 & 0.734 & 0.158 \\
BPE Whitespace (bal.) & 4.41 {\scriptsize $\pm$11.53} & 4.2929 & 0.130 & 0.406 & 0.696 & 0.815 & 0.037 \\
\bottomrule
\end{tabular}}


==> tables_camera_ready/intrinsic-flores-body.tex <==
% Body of tab:intrinsic-flores in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_intrinsic_tables.py --dataset flores --panel std1b (roster: generate_latex_tables.STD1B_MAIN_ROSTER when --panel std1b).
\small
\adjustbox{max width=\textwidth}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\textbf{Tokenizer} & \textbf{Fertility} $\downarrow$ & \textbf{Compression} $\uparrow$ & \textbf{Gini} $\downarrow$ & \textbf{Vocab CoV} $\downarrow$ & \textbf{$\bar H_2$} $\uparrow$ & \textbf{Bigram $\eta$} $\uparrow$ & \textbf{Char Split} $\downarrow$ & \textbf{AST Align} $\uparrow$ & \textbf{Digit F$_1$} $\uparrow$ & \textbf{Op Isolation} $\uparrow$ \\
\midrule
Mistral-Nemo$^\dagger$ & 4.78 & 0.0241 & 0.100 & 0.435 & 0.554 & 0.888 & 0.008 & 0.535 & 0.483 & 0.987 \\
LLaMA-3$^\dagger$ & 5.26 & 0.0185 & 0.238 & 0.447 & 0.505 & 0.822 & 0.137 & 0.511 & 0.643 & 0.987 \\
\midrule
BPE Punct (bal.) & 4.78 & 0.0215 & 0.196 & 0.495 & 0.535 & 0.843 & 0.025 & 1.000 & 0.662 & 1.000 \\
BPE Punct (eng.) & 9.39 & 0.0131 & 0.267 & 0.721 & 0.501 & 0.767 & 0.247 & 1.000 & 0.671 & 1.000 \\
BPE GPT-4o (bal.) & 4.34 & 0.0235 & 0.128 & 0.491 & 0.561 & 0.890 & 0.031 & 0.545 & 0.643 & 0.987 \\
BPE GPT-4o NFC & 4.34 & 0.0236 & 0.126 & 0.491 & 0.561 & 0.891 & 0.031 & 0.545 & 0.643 & 0.987 \\
BPE GPT-4o (eng.) & 9.57 & 0.0130 & 0.269 & 0.735 & 0.499 & 0.772 & 0.287 & 0.658 & 0.643 & 0.990 \\
BPE GPT-4o (eng., full-byte) & 9.57 & 0.0130 & 0.269 & 0.735 & 0.499 & 0.772 & 0.287 & 0.683 & 0.643 & 0.990 \\
BPE GPT-4o (code) & 7.59 & 0.0139 & 0.256 & 0.676 & 0.513 & 0.780 & 0.243 & 0.516 & 0.643 & 0.987 \\
BPE Claude (bal.) & 4.33 & 0.0237 & 0.125 & 0.486 & 0.560 & 0.889 & 0.030 & 0.748 & 0.643 & 0.997 \\
BPE Claude NFC & 4.32 & 0.0237 & 0.123 & 0.486 & 0.560 & 0.890 & 0.030 & 0.748 & 0.643 & 0.997 \\
BPE Claude (eng.) & 9.41 & 0.0132 & 0.264 & 0.734 & 0.504 & 0.774 & 0.274 & 0.787 & 0.643 & 0.997 \\
BPE RightAlign (bal.) & 4.34 & 0.0235 & 0.128 & 0.487 & 0.561 & 0.889 & 0.031 & 0.545 & 1.000 & 0.987 \\
BPE RightAlign NFC & 4.34 & 0.0236 & 0.126 & 0.487 & 0.561 & 0.890 & 0.031 & 0.545 & 1.000 & 0.987 \\
Unigram GPT-4o & 4.27 & 0.0192 & 0.121 & 0.393 & 0.324 & 0.770 & 0.049 & 0.724 & 0.483 & 1.000 \\
Unigram Claude & 4.30 & 0.0192 & 0.120 & 0.380 & 0.333 & 0.773 & 0.054 & 0.794 & 0.483 & 1.000 \\
Unigram RightAlign & 4.27 & 0.0192 & 0.121 & 0.394 & 0.324 & 0.770 & 0.049 & 0.724 & 0.483 & 1.000 \\
SuperBPE GPT-4o (bal.) & 4.40 & 0.0234 & 0.158 & 0.541 & 0.629 & 0.899 & 0.037 & 0.416 & 0.643 & 0.808 \\
PA-BPE NFC GPT-4o & 3.99 & 0.0275 & 0.017 & 0.259 & 0.540 & 0.911 & 0.015 & 0.605 & 0.633 & 0.990 \\
Unigram GPT-4o (highmid) & 4.81 & 0.0161 & 0.224 & 0.492 & 0.340 & 0.740 & 0.186 & 0.724 & 0.483 & 1.000 \\
Unigram GPT-4o (highres) & 6.48 & 0.0141 & 0.201 & 0.618 & 0.335 & 0.724 & 0.221 & 0.716 & 0.483 & 1.000 \\
MinGram SCRIPT-enc & 4.22 & 0.0244 & 0.119 & 0.478 & 0.542 & 0.891 & 0.001 & 0.748 & 0.637 & 0.997 \\
MinGram SCRIPT-enc (nl-split) & 4.22 & 0.0244 & 0.119 & 0.478 & 0.542 & 0.891 & 0.001 & 0.748 & 0.637 & 0.997 \\
BPE SCRIPT-enc GPT-4o & 4.31 & 0.0237 & 0.123 & 0.490 & 0.557 & 0.890 & 0.001 & 0.546 & 0.643 & 0.987 \\
BPE GPT-2 (bal.) & 4.76 & 0.0216 & 0.195 & 0.493 & 0.546 & 0.848 & 0.026 & 0.749 & 0.662 & 0.997 \\
BPE GPT-4o (all-eq.) & 4.07 & 0.0264 & 0.050 & 0.267 & 0.547 & 0.910 & 0.015 & 0.546 & 0.643 & 0.987 \\
BPE Claude (all-eq.) & 4.06 & 0.0265 & 0.050 & 0.259 & 0.545 & 0.909 & 0.015 & 0.748 & 0.643 & 0.997 \\
BPE Punct (all-eq.) & 4.60 & 0.0230 & 0.166 & 0.343 & 0.528 & 0.842 & 0.014 & 1.000 & 0.660 & 1.000 \\
BPE GPT-4o NFC (all-eq.) & 4.07 & 0.0265 & 0.048 & 0.267 & 0.547 & 0.912 & 0.015 & 0.546 & 0.643 & 0.987 \\
BPE GPT-4o (all-eq., no-rep.) & 4.07 & 0.0264 & 0.050 & 0.267 & 0.547 & 0.910 & 0.015 & 0.546 & 0.643 & 0.987 \\
BPE GPT-4o (bal., mf50) & 4.34 & 0.0235 & 0.128 & 0.491 & 0.561 & 0.890 & 0.031 & 0.545 & 0.643 & 0.987 \\
BPE NFC clean (bal.) & 4.33 & 0.0234 & 0.137 & 0.507 & 0.557 & 0.881 & 0.032 & 0.749 & 0.483 & 0.997 \\
BPE NFC clean plus2 (bal.) & 4.35 & 0.0235 & 0.122 & 0.498 & 0.557 & 0.883 & 0.030 & 0.749 & 0.483 & 0.997 \\
BPE NFC clean plus3 (bal.) & 4.35 & 0.0235 & 0.122 & 0.499 & 0.557 & 0.883 & 0.030 & 0.751 & 0.483 & 0.997 \\
SuperBPE PA-BPE GPT-4o & 3.99 & 0.0277 & 0.036 & 0.313 & 0.598 & 0.926 & 0.016 & 0.446 & 0.643 & 0.845 \\
SuperBPE PA-BPE GPT-4o t64k & 4.02 & 0.0271 & 0.051 & 0.355 & 0.610 & 0.926 & 0.018 & 0.425 & 0.643 & 0.815 \\
SuperBPE clean C2 (bal.) & 4.09 & 0.0269 & 0.036 & 0.328 & 0.545 & 0.908 & 0.016 & 0.734 & 0.483 & 0.997 \\
SuperBPE clean C3 (bal.) & 3.97 & 0.0277 & 0.040 & 0.326 & 0.615 & 0.928 & 0.016 & 0.517 & 0.643 & 0.838 \\
SuperBPE Punct t64k & 4.47 & 0.0232 & 0.169 & 0.535 & 0.658 & 0.898 & 0.031 & 0.445 & 0.650 & 0.391 \\
PA-BPE NFC GPT-4o HW & 3.95 & 0.0274 & 0.030 & 0.252 & 0.542 & 0.913 & 0.014 & 0.566 & 0.643 & 0.990 \\
PA-BPE NFC clean & 4.12 & 0.0266 & 0.019 & 0.276 & 0.540 & 0.898 & 0.015 & 0.752 & 0.483 & 0.997 \\
Unigram GPT-4o tuned & 4.19 & 0.0192 & 0.125 & 0.402 & 0.327 & 0.776 & 0.051 & 0.721 & 0.483 & 0.997 \\
BPE GPT-4o (highres) & 7.52 & 0.0143 & 0.309 & 0.656 & 0.484 & 0.772 & 0.268 & 0.543 & 0.643 & 0.987 \\
BPE GPT-4o (highmid) & 5.07 & 0.0180 & 0.302 & 0.526 & 0.470 & 0.807 & 0.205 & 0.545 & 0.643 & 0.987 \\
BPE Whitespace (bal.) & 4.39 & 0.0233 & 0.138 & 0.501 & 0.683 & 0.899 & 0.036 & 0.409 & 0.630 & 0.828 \\
\bottomrule
\end{tabular}}


==> tables_camera_ready/lang-breakdown-body.tex <==
% Body of tab:lang-breakdown in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
\scriptsize
\begin{tabular}{llcrrc}
\toprule
\textbf{Language} & \textbf{Code} & \textbf{Script} & \textbf{GB} & \textbf{\%} & \textbf{Docs} \\
\midrule
Russian & \texttt{rus\_Cyrl} & Cyrillic & 4.521 & 18.1 & 531,387 \\
Spanish & \texttt{spa\_Latn} & Latin & 0.423 & 1.7 & 122,231 \\
German & \texttt{deu\_Latn} & Latin & 0.353 & 1.4 & 118,340 \\
French & \texttt{fra\_Latn} & Latin & 0.364 & 1.5 & 103,496 \\
Chinese & \texttt{cmn\_Hani} & CJK & 0.326 & 1.3 & 95,805 \\
Japanese & \texttt{jpn\_Jpan} & CJK & 0.204 & 0.8 & 63,316 \\
Italian & \texttt{ita\_Latn} & Latin & 0.165 & 0.7 & 59,676 \\
Portuguese & \texttt{por\_Latn} & Latin & 0.189 & 0.8 & 59,460 \\
Turkish & \texttt{tur\_Latn} & Latin & 0.152 & 0.6 & 47,074 \\
Indonesian & \texttt{ind\_Latn} & Latin & 0.236 & 0.9 & 45,970 \\
Polish & \texttt{pol\_Latn} & Latin & 0.107 & 0.4 & 43,902 \\
Ukrainian & \texttt{ukr\_Cyrl} & Cyrillic & 0.211 & 0.8 & 34,088 \\
Dutch & \texttt{nld\_Latn} & Latin & 0.071 & 0.3 & 32,404 \\
Romanian & \texttt{ron\_Latn} & Latin & 0.097 & 0.4 & 29,203 \\
Arabic & \texttt{arb\_Arab} & Arabic & 0.168 & 0.7 & 27,292 \\
Hungarian & \texttt{hun\_Latn} & Latin & 0.099 & 0.4 & 25,066 \\
Vietnamese & \texttt{vie\_Latn} & Latin & 0.109 & 0.4 & 21,306 \\
Czech & \texttt{ces\_Latn} & Latin & 0.077 & 0.3 & 21,696 \\
Greek & \texttt{ell\_Grek} & Greek & 0.108 & 0.4 & 17,672 \\
Thai & \texttt{tha\_Thai} & Thai & 0.087 & 0.3 & 11,639 \\
Finnish & \texttt{fin\_Latn} & Latin & 0.034 & 0.1 & 11,721 \\
Slovak & \texttt{slk\_Latn} & Latin & 0.028 & 0.1 & 10,015 \\
Bulgarian & \texttt{bul\_Cyrl} & Cyrillic & 0.052 & 0.2 & 9,513 \\
Korean & \texttt{kor\_Hang} & Hangul & 0.029 & 0.1 & 8,263 \\
Croatian & \texttt{hrv\_Latn} & Latin & 0.026 & 0.1 & 8,395 \\
Catalan & \texttt{cat\_Latn} & Latin & 0.014 & 0.1 & 5,087 \\
Hindi & \texttt{hin\_Deva} & Devanagari & 0.032 & 0.1 & 4,928 \\
Hebrew & \texttt{heb\_Hebr} & Hebrew & 0.025 & 0.1 & 4,665 \\
Bengali & \texttt{ben\_Beng} & Bengali & 0.024 & 0.1 & 3,525 \\
Tamil & \texttt{tam\_Taml} & Tamil & 0.017 & 0.1 & 1,831 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/main-results-body.tex <==
% Body of tab:main-results in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_latex_tables.py --table main (roster/columns: results/paper_subset_recommendation_2026-08-09.md S1/S3; Code BPB column removed 2026-08-10, see tab:cross-regime-code-bpb).
\small
\begin{tabular}{l c cc cc cc}
\toprule
 & \multicolumn{5}{c}{\textbf{Perplexity $\downarrow$} (mean $|$ cross-language $\sigma$)} & \multicolumn{2}{c}{\textbf{Ling.} $\uparrow$} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-8}
\textbf{Tokenizer} & \textbf{Val} & \textbf{FLORES (tr.)} & \textbf{$\sigma$} & \textbf{FLORES (all)} & \textbf{$\sigma$} & \textbf{BLiMP} & \textbf{MultiBLiMP} \\
\midrule
Mistral-Nemo$^\dagger$ & 0.7212 & 1.173 & 0.299 & 2.756 & 1.012 & 0.817 & 0.915 \\
LLaMA-3$^\dagger$ & 0.7198 & 1.173 & 0.293 & 2.662 & 1.014 & 0.826 & 0.914 \\
\midrule
BPE Punct (bal.) & 0.7185 & 1.167 & 0.291 & 2.647 & 1.018 & 0.817 & 0.913 \\
BPE Punct (eng.) & 0.7360 & 1.191 & 0.308 & 2.636 & 1.015 & 0.807 & 0.911 \\
BPE GPT-4o (bal.) & 0.7131 & 1.161 & 0.294 & 2.641 & 1.020 & 0.820 & 0.916 \\
BPE GPT-4o NFC & 0.7133 & 1.159 & 0.298 & 2.638 & 1.019 & 0.820 & 0.920 \\
BPE GPT-4o (eng.) & 0.7375 & 1.197 & 0.312 & 2.638 & 1.015 & 0.807 & 0.911 \\
BPE GPT-4o (eng., full-byte) & 0.7382 & 1.201 & 0.316 & 2.644 & 1.017 & 0.817 & 0.912 \\
BPE GPT-4o (code) & 0.7252 & 1.179 & 0.295 & 2.626 & 1.009 & 0.819 & 0.913 \\
BPE Claude (bal.) & 0.7156 & 1.162 & 0.296 & 2.642 & 1.016 & 0.816 & 0.914 \\
BPE Claude NFC & 0.7152 & 1.159 & 0.300 & 2.642 & 1.018 & 0.819 & 0.911 \\
BPE Claude (eng.) & 0.7330 & 1.194 & 0.311 & 2.641 & 1.021 & 0.817 & 0.907 \\
BPE RightAlign (bal.) & 0.7138 & 1.164 & 0.293 & 2.641 & 1.016 & 0.813 & 0.909 \\
BPE RightAlign NFC & 0.7138 & 1.161 & 0.298 & 2.642 & 1.018 & 0.816 & 0.911 \\
Unigram GPT-4o & 0.7338 & 1.193 & 0.304 & 2.687 & 1.010 & 0.834 & 0.903 \\
Unigram Claude & 0.7359 & 1.189 & 0.302 & 2.683 & 1.007 & 0.841 & 0.905 \\
Unigram RightAlign & 0.7338 & 1.193 & 0.302 & 2.684 & 1.002 & 0.828 & 0.908 \\
SuperBPE GPT-4o (bal.) & 0.7236 & 1.173 & 0.297 & 2.639 & 1.013 & 0.804 & 0.909 \\
PA-BPE NFC GPT-4o & 0.7255 & 1.186 & 0.300 & 2.662 & 1.006 & 0.817 & 0.904 \\
Unigram GPT-4o (highmid) & 0.7345 & 1.197 & 0.306 & 2.675 & 1.003 & 0.831 & 0.913 \\
Unigram GPT-4o (highres) & 0.7305 & 1.197 & 0.305 & 2.666 & 0.994 & 0.824 & 0.907 \\
MinGram SCRIPT-enc & 0.7129 & 1.165 & 0.303 & 2.685 & 1.048 & 0.813 & 0.920 \\
MinGram SCRIPT-enc (nl-split) & 0.7134 & 1.159 & 0.301 & 2.671 & 1.058 & 0.815 & 0.918 \\
BPE SCRIPT-enc GPT-4o & 0.7128 & 1.157 & 0.297 & 2.657 & 1.046 & 0.822 & 0.916 \\
BPE GPT-2 (bal.) & 0.7128 & 1.157 & 0.287 & 2.635 & 1.016 & 0.816 & 0.910 \\
BPE GPT-4o (all-eq.) & 0.7177 & 1.172 & 0.292 & 2.652 & 1.016 & 0.819 & 0.918 \\
BPE Claude (all-eq.) & 0.7200 & 1.170 & 0.291 & 2.654 & 1.015 & 0.817 & 0.921 \\
BPE Punct (all-eq.) & 0.7223 & 1.168 & 0.294 & 2.648 & 1.019 & 0.818 & 0.917 \\
BPE GPT-4o NFC (all-eq.) & 0.7165 & 1.164 & 0.295 & 2.646 & 1.014 & 0.823 & 0.917 \\
BPE GPT-4o (all-eq., no-rep.) & 0.7165 & 1.168 & 0.292 & 2.648 & 1.015 & 0.819 & 0.913 \\
BPE GPT-4o (bal., mf50) & 0.7116 & 1.158 & 0.292 & 2.629 & 1.013 & 0.822 & -- \\
BPE NFC clean (bal.) & 0.7159 & 1.157 & 0.296 & 2.648 & 1.022 & 0.821 & 0.910 \\
BPE NFC clean plus2 (bal.) & 0.7162 & 1.158 & 0.297 & 2.638 & 1.017 & 0.814 & 0.918 \\
BPE NFC clean plus3 (bal.) & 0.7149 & 1.155 & 0.297 & 2.635 & 1.017 & 0.818 & 0.918 \\
SuperBPE PA-BPE GPT-4o & 0.7292 & 1.181 & 0.294 & 2.653 & 1.008 & 0.801 & 0.916 \\
SuperBPE PA-BPE GPT-4o t64k & 0.7293 & 1.181 & 0.295 & 2.652 & 1.011 & 0.792 & 0.920 \\
SuperBPE clean C2 (bal.) & 0.7285 & 1.169 & 0.293 & 2.650 & 1.011 & 0.811 & 0.912 \\
SuperBPE clean C3 (bal.) & 0.7296 & 1.174 & 0.294 & 2.644 & 1.006 & 0.803 & 0.919 \\
SuperBPE Punct t64k & 0.7259 & 1.167 & 0.293 & 2.630 & 1.009 & 0.808 & 0.915 \\
PA-BPE NFC GPT-4o HW & 0.7194 & 1.177 & 0.299 & 2.656 & 1.007 & 0.816 & 0.914 \\
PA-BPE NFC clean & 0.7235 & 1.178 & 0.302 & 2.653 & 1.007 & 0.819 & 0.907 \\
Unigram GPT-4o tuned & 0.7333 & 1.192 & 0.302 & 2.686 & 1.009 & 0.838 & 0.912 \\
BPE GPT-4o (highres) & 0.7127 & 1.182 & 0.294 & 2.618 & 0.999 & 0.814 & 0.912 \\
BPE GPT-4o (highmid) & 0.7137 & 1.174 & 0.296 & 2.637 & 1.016 & 0.815 & 0.910 \\
BPE Whitespace (bal.) & 0.7207 & 1.165 & 0.294 & 2.622 & 1.003 & 0.814 & 0.915 \\
Unigram Whitespace tuned (bal.) & 0.8401 & 1.176 & 0.298 & 2.576 & 0.949 & 0.805 & 0.918 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/mc20b-results-body.tex <==
% Body of tab:mc20b-results in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_latex_tables.py --table mc20b (roster: configs/panels/panels.json 'mc20b_extended_v20260811', EXPERIMENTAL_SETUP.md 'Panel redesign 2026-08-11'). $^{b}$ marks the E4 initial_alphabet byte-drop defect on the rows in MC20B_DEFECT_FLAGGED (claude-english-bpe and, since the 2026-08-17 disclosure ruling, punct-english-bpe); $^{e}$ marks the 4 extended-only rows (MC20B_EXTENDED_ONLY, not members of the 20-member correlation panel mc20b_primary_v20260811); the caption text for footnotes b and e is hand-maintained in the main tex, not regenerated here.
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Tokenizer} & \textbf{MBPP} & \textbf{HumanEval} & \textbf{GSM8K} & \textbf{Code BPB} \\
\midrule
BPE Punct (bal.) & 0.230 & 0.171 & 0.189 & 0.380 \\
BPE Punct (eng.)$^{b}$ & 0.228 & 0.165 & 0.208 & 0.372 \\
BPE GPT-4o (bal.) & 0.174 & 0.165 & 0.198 & 0.377 \\
BPE GPT-4o NFC & 0.120 & 0.152 & 0.208 & 0.379 \\
BPE GPT-4o (eng., full-byte) & 0.064 & 0.152 & 0.218 & 0.399 \\
BPE GPT-4o (code) & 0.016 & 0.159 & 0.216 & 0.380 \\
BPE Claude (bal.) & 0.250 & 0.171 & 0.227 & 0.386 \\
BPE Claude NFC & 0.224 & 0.159 & 0.230 & 0.385 \\
BPE Claude (eng.)$^{b}$ & 0.234 & 0.165 & 0.221 & 0.365 \\
BPE RightAlign (bal.) & 0.072 & 0.152 & 0.234 & 0.380 \\
BPE RightAlign NFC & 0.104 & 0.171 & 0.224 & 0.381 \\
Unigram GPT-4o & 0.000 & 0.134 & 0.187 & 0.399 \\
Unigram Claude & 0.222 & 0.146 & 0.165 & 0.403 \\
Unigram RightAlign & 0.000 & 0.140 & 0.175 & 0.399 \\
SuperBPE GPT-4o (bal.) & 0.068 & 0.159 & 0.180 & 0.383 \\
PA-BPE NFC GPT-4o & 0.130 & 0.165 & 0.203 & 0.388 \\
MinGram SCRIPT-enc & 0.016 & 0.177 & 0.199 & 0.379 \\
BPE SCRIPT-enc GPT-4o & 0.136 & 0.171 & 0.205 & 0.378 \\
BPE NFC clean (bal.) & 0.218 & 0.159 & 0.177 & 0.381 \\
SuperBPE clean C2 (bal.) & 0.202 & 0.134 & 0.241 & 0.391 \\
\crnew{BPE NFC clean plus2 (bal.)}$^{e}$ & 0.114 & 0.152 & 0.212 & 0.379 \\
\crnew{BPE NFC clean plus3 (bal.)}$^{e}$ & 0.220 & 0.171 & 0.197 & 0.383 \\
\crnew{SuperBPE clean C3 (bal.)}$^{e}$ & 0.190 & 0.140 & 0.171 & 0.390 \\
\crnew{MinGram SCRIPT-enc (nl-split)}$^{e}$ & 0.216 & 0.152 & 0.235 & 0.383 \\
\midrule
Mistral-Nemo$^\dagger$ & 0.000 & 0.152 & 0.184 & 0.378 \\
LLaMA-3$^\dagger$ & 0.082 & 0.171 & 0.233 & 0.378 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/metric-summary-body.tex <==
% Body of tab:metric-summary in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
\small
\adjustbox{max width=\textwidth}{%
\begin{tabular}{@{}p{3.3cm}p{5.5cm}p{6.8cm}@{}}
\toprule
\textbf{Metric} & \textbf{Formula} & \textbf{Interpretation} \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Compression \& Information-Theoretic} (\cref{sec:compression})} \\[2pt]
Compression rate & $\mathrm{CR}_\ell = \sum_{i:\ell_i=\ell} |\inputtext_i|_u \,/\, \sum_{i:\ell_i=\ell} |\toksequence_i|$ & Multiplier by which tokenization compresses. $\uparrow$ = more compression. \\
Unigram entropy & $H(p(\cdot)) = -\sum_t p(t) \log_2 p(t)$ & Uniformity of vocabulary usage. $\uparrow$ = more even. \\
% ADDED 2026-08-17 (consistency pass): vocabulary utilization and token length are defined in
% Section 3.1 and appear in the results tables (vocab.\ utilization in tab:aggregate-correlations,
% tab:mixed-effects, tab:heldout-reference; token length as a selected predictor in
% tab:heldout-reference), but had no row here.
Vocab.\ utilization & $|\{t \in \vocab : p(t) > 0\}| \,/\, |\vocab|$ & Fraction of vocabulary entries the corpus uses at least once. \\
Token length & $\sum_{i}|\inputtext_i|_{\texttt{chars}} \,/\, \sum_i |\toksequence_i|$ & Mean characters per token occurrence. \\[5pt]
% AUDIT 2026-08-07: point 1. The implemented normalizer is $\log_2$ of the number of
% distinct successors the context itself had, not $\log_2|\vocab|$.
Bigram entropy & $\eta(t) = H(p(\cdot|t))\, / \,\log_2 |\mathcal{A}(t)|$; \newline $\bar\eta = \sum_t n_t\eta(t)/\sum_t n_t$ & Conditional entropy of the next token given the previous one, divided by the entropy the context's own observed successor set could carry. $\bar\eta \!\in\! [0,1]$; $\downarrow$ = predictable sequences. \\[15pt]
% AUDIT 2026-08-07: point 6. The implemented $\alpha$ set is $\{1,2,2.5,3\}$.
R\'enyi efficiency & $\bar H_\alpha(p(\cdot)) = H_\alpha(p(\cdot)) / \log_2|\vocab|$, \newline $H_\alpha(p(\cdot)) = \frac{1}{1-\alpha}\log_2(\sum_t p(t)^\alpha)$ & Generalized uniformity; computed for $\alpha \in \{1,2,2.5,3\}$, and reported here for $\alpha=2$. $\uparrow$ = more uniform token usage. \\[20pt]
% AUDIT 2026-08-07: point 10. State the ranking domain: $r$ ranks the types observed in the
% corpus, not the declared vocabulary.
Avg.\ token rank & $\bar{r}_\ell = \sum_{i:\ell_i=\ell}\sum_j r(t_{i,j}) \,/\, \sum_{i:\ell_i=\ell} |\toksequence_i|$ &Token frequency rank averaged over all token occurrences, where $r$ ranks by frequency in the corpus. $\downarrow$ = few common tokens dominate. \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Linguistic Alignment} (\cref{sec:linguistic})} \\[2pt]
Fertility & $\mathrm{Fert}_\ell = \text{mean}_{i:\ell_i=\ell}\, |\toksequence_i|/|\inputtext_i|_{\texttt{words}}$ & Tokens per word; default $u{=}\texttt{words}$ (mean of ratios). $1.0$ = one token per word. \\
MorphScore & Morpheme boundary P/R/F1 (external library) & Token--morpheme alignment across 70 languages. \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Multilingual Fairness} (\cref{sec:fairness})} \\[2pt]
TFG (Gini) & $\mathrm{TFG} = \sum_{i,j}|c_i - c_j| \,/\, 2n^2\mu$, \newline $c_\ell = \sum_i|\toksequence_i|/\sum_i|\inputtext_i|_u$ & Cross-lingual inequality of tokenization cost. $0$ = perfect parity. $n =$  number of languages; $\mu=$ mean of per-language costs $c_\ell$ \\[10pt]
Vocab.\ util.\ CoV & $u_\ell = |\{\text{used vocab entries in }\ell\}| / |\vocab|$; \newline $\mathrm{CoV} = \sigma(u_\ell)/\mu(u_\ell)$ over languages $\ell$ & Cross-lingual dispersion of per-language vocabulary utilization ($\mu$ = mean, $\sigma$ = sample std). $\downarrow$ = similar utilization across languages. \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Encoding Fidelity} (\cref{sec:fidelity})} \\[2pt]
Exact match & $\mathbb{1}[\hat{\inputtext} = \inputtext]$, averaged over corpus & Strict round-trip reconstruction rate. \\
CER & $\mathrm{Lev}(\inputtext, \hat{\inputtext})\,/\,|\inputtext|_{\texttt{chars}}$ & Character-level Levenshtein distance, normalized; can exceed 1. \\
% AUDIT 2026-08-07: point 2. The quantity is computed over token OCCURRENCES in the corpus,
% not over the vocabulary.
UTF-8 completeness & $|\{(i,j): \text{bytes}(t_{i,j})\,  \text{is  valid UTF-8 and }\, t_{i,j} \notin \mathcal{S}\}|/ |\{(i,j): t_{i,j} \notin \mathcal{S}\}$ & Fraction of non-special token occurrences that decode to complete characters. Occurrence-weighted in the corpus. \\
Char split rate & $|\{c : \text{multi-byte, split}\}| \,/\, |\{c : \text{multi-byte}\}|$ & Proportion of multi-byte chars whose bytes span multiple tokens. \\
% ADDED 2026-08-17 (consistency pass): defined in Section 3.4 and reported in
% tab:aggregate-correlations and tab:mixed-effects, but had no row here.
UTF-8 boundary crossing & Frac.\ of non-special token occurrences spanning $>$1 character and leaving one of them incomplete & Frequency of tokens produced by a merge across a character boundary. \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Digit Tokenization} (\cref{sec:math-metrics})} \\[2pt]
Digit boundary $F_1$ & $F_1$ of $B_{\mathrm{obs}}$ vs.\ $B_{\mathrm{ideal}}$ (right-aligned triples) & Place-value alignment of digit span segmentation. \\
Digit split variability & $H_{\mathrm{pattern}} = -\sum_p (n_p/N)\log_2(n_p/N)$ & Entropy of splitting patterns for same-length digit spans. $\downarrow$ = consistent. \\
% AUDIT 2026-08-07: point 3. The implemented rule allows a covering token to carry
% whitespace; only non-whitespace characters from outside the operator span break isolation.
Operator isolation & Frac.\ of operator occurrences whose covering tokens carry no non-whitespace character from outside the operator span & Whether operators are fused with adjacent operands. Computed separately on prose, code and math; reported here on the math corpus. \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Code Tokenization} (\cref{sec:code-metrics})} \\[2pt]
AST boundary alignment & Frac.\ of AST leaf nodes fully aligned with token boundaries & Per-category (identifier, keyword, operator, literal, delimiter). \\
Ident.\ fragmentation & Frac.\ of identifiers split across $>$1 token & $\uparrow$ = more fragmentation of programmer-defined names. \\
% ADDED 2026-08-17 (consistency pass): both are selected predictors in tab:heldout-reference.
%Tokens per identifier & Mean token count per identifier occurrence & As ident.\ fragmentation, graded rather than binary. \\
%End-alignment rate & Frac.\ of AST leaf nodes whose end offset falls on a token boundary & One-sided form of AST boundary alignment. \\
Indentation consistency & $\rho(\text{nesting depth}, \text{whitespace token count})$ & Spearman correlation; $\uparrow$ = more monotonic increase in token count for more whitespace. \\
\bottomrule
\end{tabular}}




==> tables_camera_ready/mixed-effects-body.tex <==
% Body of tab:mixed-effects in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Combined FLORES-BPB + MultiBLiMP-accuracy table (2026-08-12 fix-list ruling: merged, no separate MultiBLiMP table).
% Stars/bold and the printed +/-SE come from the family-clustered inference (p_adj_clustered / std_error_clustered; 2026-08-14 user ruling). The MixedLM beta is unchanged; naive columns remain in the CSVs.
% FLORES arm: n_obs=899, n_languages=31. MultiBLiMP arm: n_obs=696, n_languages=24. Keep the caption's stated n's in sync with these (hand-maintained, not auto-inserted).
\small
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Intrinsic Metric}} & \multicolumn{2}{c}{\textbf{FLORES BPB}} & \multicolumn{2}{c}{\textbf{MultiBLiMP acc.}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & $\beta$ & $\tilde{\rho}$ & $\beta$ & $\tilde{\rho}$ \\
\midrule
Fertility & $\textbf{+0.018}^{***}${\scriptsize$\pm$0.004} & $\textbf{+0.385}$ & $-0.004${\scriptsize$\pm$0.002} & $+0.060$ \\
UTF-8 char split & $\textbf{+0.014}^{***}${\scriptsize$\pm$0.002} & $\textbf{+0.484}$ & $\textbf{-0.005}^{*}${\scriptsize$\pm$0.002} & $\textbf{-0.068}$ \\
Trigram entropy & $\textbf{-0.013}^{***}${\scriptsize$\pm$0.002} & $\textbf{-0.463}$ & $\textbf{+0.003}^{*}${\scriptsize$\pm$0.001} & $\textbf{-0.001}$ \\
Bigram entropy & $\textbf{-0.011}^{***}${\scriptsize$\pm$0.002} & $\textbf{-0.375}$ & $\textbf{+0.003}^{*}${\scriptsize$\pm$0.001} & $\textbf{+0.017}$ \\
Compression rate & $\textbf{-0.010}^{***}${\scriptsize$\pm$0.003} & $\textbf{-0.385}$ & $+0.002${\scriptsize$\pm$0.002} & $-0.063$ \\
R\'enyi eff.\ ($\alpha$=2) & $\textbf{-0.010}^{***}${\scriptsize$\pm$0.001} & $\textbf{-0.378}$ & $\textbf{+0.003}^{*}${\scriptsize$\pm$0.001} & $\textbf{+0.134}$ \\
Unigram entropy & $\textbf{-0.010}^{***}${\scriptsize$\pm$0.002} & $\textbf{-0.326}$ & $+0.002${\scriptsize$\pm$0.001} & $-0.163$ \\
UTF-8 boundary crossing & $\textbf{+0.004}^{*}${\scriptsize$\pm$0.001} & $\textbf{+0.360}$ & $\textbf{-0.005}^{*}${\scriptsize$\pm$0.001} & $\textbf{+0.003}$ \\
Vocab utilization & $-0.002${\scriptsize$\pm$0.004} & $-0.191$ & $-0.001${\scriptsize$\pm$0.002} & $-0.122$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/optimizer-body.tex <==
% Body of tab:optimizer in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
\small
\begin{tabular}{lllcl}
\toprule
\textbf{Group} & \textbf{Optimizer} & \textbf{Eff.\ LR} & \textbf{Betas} & \textbf{WD} \\
\midrule
Transformer matrices & Muon & 0.0283 & mom.\ schedule & 0.050$\to$0 \\
Input embeddings & AdamW & 0.2121 & (0.8, 0.995) & 0.001 \\
Output projection & AdamW & 0.0057 & (0.8, 0.96) & 0.01 \\
Value embeddings & AdamW & 0.1061 & (0.8, 0.995) & 0.01 \\
Residual scalars & AdamW & 0.0071 & (0.8, 0.95) & 0.05 \\
Skip scalars & AdamW & 0.707 & (0.96, 0.95) & 0.0 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/pairwise-compact-body.tex <==
% Body of tab:pairwise-compact in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
\small
\begin{tabular}{llllllcc}
\toprule
\textbf{Factor} & \textbf{A} & \textbf{B} & $\Delta$\textbf{Val} & $\Delta$\textbf{FLORES (tr.)} & $\Delta$\textbf{FLORES (all)} & $\Delta$\textbf{BLiMP} & $\Delta$\textbf{Code} \\
\midrule
\multirow{3}{*}{NFC normalization} & GPT-4o & + NFC & $+0.0004$ & $-0.0020$ & $\textbf{-0.0033}$ & $+0.0006$ & $+0.0002$ \\
 & Claude & + NFC & $\textbf{-0.0012}$ & $-0.0033$ & $-0.0001$ & $+0.0026$ & $+0.0004$ \\
 & RightAlign & + NFC & $\textbf{-0.0007}$ & $-0.0028$ & $+0.0007$ & $+0.0026$ & $+0.0002$ \\
\midrule
\multirow{3}{*}{Algorithm} & BPE GPT-4o & Unigram & $\textbf{+0.0331}$ & $\textbf{+0.0323}$ & $\textbf{+0.0464}$ & $+0.0142$ & $+0.0364$ \\
 & BPE Claude & Unigram & $\textbf{+0.0304}$ & $\textbf{+0.0266}$ & $\textbf{+0.0414}$ & $+0.0244$ & $+0.0375$ \\
 & BPE RightAlign & Unigram & $\textbf{+0.0300}$ & $\textbf{+0.0290}$ & $\textbf{+0.0432}$ & $+0.0146$ & $+0.0343$ \\
\midrule
\multirow{1}{*}{Unigram tuning} & Untuned & Tuned & $\textbf{+0.0033}$ & $-0.0010$ & $-0.0010$ & $+0.0042$ & $-0.0004$ \\
\midrule
\multirow{5}{*}{Pretokenizer} & GPT-4o & Claude & $\textbf{+0.0019}$ & $+0.0014$ & $+0.0007$ & $-0.0033$ & $-0.0003$ \\
 & GPT-4o & Punct & $\textbf{+0.0074}$ & $\textbf{+0.0057}$ & $\textbf{+0.0059}$ & $-0.0026$ & $+0.0097$ \\
 & GPT-4o & RightAlign & $\textbf{+0.0021}$ & $\textbf{+0.0028}$ & $+0.0000$ & $-0.0065$ & $+0.0018$ \\
 & GPT-4o & Whitespace & $\textbf{+0.0115}$ & $\textbf{+0.0037}$ & $\textbf{-0.0196}$ & $-0.0060$ & $+0.0064$ \\
 & GPT-4o & GPT-2 & $\textbf{+0.0052}$ & $\textbf{-0.0034}$ & $\textbf{-0.0062}$ & $-0.0039$ & $-0.0051$ \\
\midrule
\multirow{6}{*}{Training data} & Balanced & English & $\textbf{+0.0511}$ & $\textbf{+0.0364}$ & $-0.0025$ & $-0.0131$ & $+0.0361$ \\
 & Balanced & Code & $\textbf{+0.0363}$ & $\textbf{+0.0182}$ & $\textbf{-0.0153}$ & $-0.0006$ & $+0.0241$ \\
 & Claude bal & Claude eng & $\textbf{+0.0475}$ & $\textbf{+0.0315}$ & $-0.0006$ & $+0.0005$ & $+0.0223$ \\
 & Punct bal & Punct eng & $\textbf{+0.0419}$ & $\textbf{+0.0245}$ & $\textbf{-0.0107}$ & $-0.0098$ & $+0.0248$ \\
 & Balanced & High-res & $\textbf{+0.0356}$ & $\textbf{+0.0216}$ & $\textbf{-0.0232}$ & $-0.0059$ & $+0.0011$ \\
 & Balanced & High-mid & $\textbf{+0.0202}$ & $\textbf{+0.0129}$ & $-0.0035$ & $-0.0047$ & $+0.0008$ \\
\midrule
\multirow{2}{*}{PA-BPE family} & GPT-4 pretok & clean pretok & $\textbf{-0.0034}$ & $\textbf{-0.0079}$ & $\textbf{-0.0089}$ & $+0.0018$ & $-0.0060$ \\
 & Base & Hybrid-window & $\textbf{-0.0095}$ & $\textbf{-0.0090}$ & $\textbf{-0.0062}$ & $-0.0006$ & $-0.0095$ \\
\midrule
\multirow{1}{*}{Trainer (BPE vs PA-BPE)} & BPE clean & PA-BPE clean & $\textbf{+0.0123}$ & $\textbf{+0.0213}$ & $+0.0052$ & $-0.0025$ & $+0.0048$ \\
\midrule
\multirow{4}{*}{SuperBPE} & GPT-4o BPE & + SuperBPE & $\textbf{+0.0069}$ & $\textbf{+0.0122}$ & $-0.0016$ & $-0.0161$ & $+0.0044$ \\
 & PA-BPE bal & + SuperBPE & $\textbf{-0.0069}$ & $-0.0049$ & $\textbf{-0.0093}$ & $-0.0154$ & $-0.0059$ \\
 & t90k & t64k & $-0.0028$ & $-0.0005$ & $-0.0004$ & $-0.0095$ & $+0.0022$ \\
 & C2 (bal) & C3 (bal) & $\textbf{+0.0019}$ & $\textbf{+0.0042}$ & $\textbf{-0.0064}$ & $-0.0084$ & $+0.0047$ \\
\bottomrule
\end{tabular}


==> tables_camera_ready/pilot-results-body.tex <==
% Body of tab:pilot-results in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained. Generated by scripts/generate_latex_tables.py --table pilot.
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Tokenizer} & \textbf{Val BPB} & \textbf{FLORES (tr.)} & \textbf{FLORES (all)} & \textbf{Code BPB} \\
\midrule
Mistral-Nemo$^\dagger$ & 0.8210 & 1.292 & 2.827 & 0.612 \\
LLaMA-3$^\dagger$ & 0.8193 & 1.304 & 2.751 & 0.622 \\
\midrule
BPE Punct (bal.) & 0.8179 & 1.295 & 2.737 & 0.613 \\
BPE Punct (eng.) & 0.8334 & 1.343 & 2.748 & 0.646 \\
BPE GPT-4o (bal.) & 0.8067 & 1.290 & 2.734 & 0.599 \\
BPE GPT-4o NFC & 0.8064 & 1.287 & 2.740 & 0.599 \\
BPE GPT-4o (eng.) & 0.8327 & 1.344 & 2.749 & 0.648 \\
BPE GPT-4o (code) & 0.8282 & 1.332 & 2.737 & 0.625 \\
BPE Claude (bal.) & 0.8131 & 1.291 & 2.740 & 0.599 \\
BPE Claude NFC & 0.8138 & 1.288 & 2.736 & 0.602 \\
BPE Claude (eng.) & 0.8327 & 1.343 & 2.748 & 0.639 \\
BPE RightAlign (bal.) & 0.8066 & 1.289 & 2.736 & 0.599 \\
BPE RightAlign NFC & 0.8065 & 1.286 & 2.734 & 0.599 \\
Unigram GPT-4o & 0.8407 & 1.328 & 2.786 & 0.642 \\
Unigram Claude & 0.8471 & 1.334 & 2.791 & 0.643 \\
Unigram RightAlign & 0.8408 & 1.326 & 2.790 & 0.642 \\
PA-BPE NFC GPT-4o & 0.8333 & 1.299 & 2.760 & 0.624 \\
PA-BPE NFC clean & 0.8309 & 1.294 & 2.752 & 0.614 \\
BPE Whitespace (bal.) & 0.8101 & 1.297 & 2.725 & 0.603 \\
BPE GPT-2 (bal.) & 0.8083 & 1.292 & 2.730 & 0.596 \\
BPE GPT-4o (highres) & 0.8084 & 1.323 & 2.721 & 0.603 \\
BPE GPT-4o (highmid) & 0.8053 & 1.300 & 2.728 & 0.598 \\
Unigram GPT-4o tuned & 0.8440 & 1.335 & 2.801 & 0.644 \\
Unigram Whitespace tuned (bal.) & 0.9633 & 1.312 & 2.692 & 0.720 \\
PA-BPE NFC GPT-4o HW & 0.8165 & 1.280 & 2.737 & 0.606 \\
SuperBPE Punct t64k & 0.8127 & 1.298 & 2.720 & 0.594 \\
SuperBPE GPT-4o (bal.) & 0.8098 & 1.302 & 2.729 & 0.592 \\
SuperBPE PA-BPE GPT-4o & 0.8214 & 1.291 & 2.742 & 0.607 \\
SuperBPE PA-BPE GPT-4o t64k & 0.8191 & 1.293 & 2.742 & 0.600 \\
SuperBPE clean C2 (bal.) & 0.8262 & 1.279 & 2.734 & 0.607 \\
SuperBPE clean C3 (bal.) & 0.8214 & 1.283 & 2.737 & 0.609 \\
BPE NFC clean (bal.) & 0.8165 & 1.286 & 2.740 & 0.605 \\
\bottomrule
\end{tabular}


==> tables_camera_ready/pretok-alphabet-controls-body.tex <==
% Body of tab:pretok-alphabet-controls in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% Generated by scripts/generate_ablation_std1b_tables.py. DO NOT EDIT BY HAND.
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Tokenizer} & \textbf{Val BPB} & \textbf{FLORES (tr.\ mean)} & \textbf{BLiMP} & \textbf{Code BPB} \\
\midrule
\texttt{gpt2-balanced-bpe} & $0.7128$ & $1.1574$ & $0.8158$ & $0.5154$ \\
\texttt{whitespace-balanced-bpe} & $0.7207$ & $1.1646$ & $0.8136$ & $0.5269$ \\
\texttt{whitespace-balanced-unigram} & $0.8401$ & $1.1756$ & $0.8052$ & $0.6091$ \\
\texttt{whitespace-multiheavy-bpe} & $0.7201$ & $1.1647$ & $0.8090$ & $0.5272$ \\
\texttt{gpt4o-english-fullbyte-bpe} & $0.7382$ & $1.2014$ & $0.8168$ & $0.5568$ \\
\texttt{clauderev-balanced-bpe}$^\dagger$ & -- & -- & $0.8198$ & -- \\
\bottomrule
\end{tabular}


==> tables_camera_ready/tokenizer-grid-body.tex <==
\textbf{Tokenizer} & \textbf{Algorithm} & \textbf{Pretok} & \textbf{Data} & \textbf{NFC} & \textbf{Panels} & \textbf{Fam.} & \textbf{Note} \\
\midrule
\endfirsthead
\toprule
\textbf{Tokenizer} & \textbf{Algorithm} & \textbf{Pretok} & \textbf{Data} & \textbf{NFC} & \textbf{Panels} & \textbf{Fam.} & \textbf{Note} \\
\midrule
\multicolumn{8}{l}{\small\itshape (continued from previous page)} \\
\midrule
\endhead
\midrule
\multicolumn{8}{r}{\small\itshape continued on next page} \\
\endfoot
\bottomrule
\endlastfoot
Mistral-Nemo & BPE & G & -- & -- & R & -- &  \\
LLaMA-3 & BPE & -- & -- & -- & R & -- &  \\
\midrule
BPE Punct (bal.) & BPE & P & B & \xmark & P, M & 1 &  \\
BPE Punct (eng.) & BPE & P & E & \xmark & P, M & 2 & incomplete byte alphabet \\
BPE GPT-4o (bal.) & BPE & G & B & \xmark & P, M & 3 &  \\
BPE GPT-4o NFC & BPE & G & B & \cmark & P, M & 4 &  \\
BPE GPT-4o (eng.) & BPE & G & E & \xmark & -- & -- & incomplete byte alphabet \\
BPE GPT-4o (eng., full-byte) & BPE & G & E & \xmark & P, M & 5 & full byte alphabet \\
BPE GPT-4o (code) & BPE & G & Co & \xmark & P, M & 6 &  \\
BPE Claude (bal.) & BPE & C & B & \xmark & P, M & 7 &  \\
BPE Claude NFC & BPE & C & B & \cmark & P, M & 8 &  \\
BPE Claude (eng.) & BPE & C & E & \xmark & M & -- & incomplete byte alphabet \\
BPE RightAlign (bal.) & BPE & R & B & \xmark & P, M & 9 &  \\
BPE RightAlign NFC & BPE & R & B & \cmark & P, M & 10 &  \\
Unigram GPT-4o & Unigram & G & B & \xmark & P, M & 11 &  \\
Unigram Claude & Unigram & C & B & \xmark & P, M & 12 &  \\
Unigram RightAlign & Unigram & R & B & \xmark & P, M & 13 &  \\
SuperBPE GPT-4o (bal.) & SuperBPE & G & B & \xmark & P, M & 14 &  \\
PA-BPE NFC GPT-4o & PA-BPE & G & B & \cmark & P, M & 15 &  \\
Unigram GPT-4o (highmid) & Unigram & G & Hm & \xmark & P & 16 & 21 langs \\
Unigram GPT-4o (highres) & Unigram & G & Hr & \xmark & P & 17 & 6 langs \\
MinGram SCRIPT-enc & MinGram & S & B & \cmark & P, M & 18 & SCRIPT enc. \\
MinGram SCRIPT-enc (nl-split) & MinGram & S & B & \cmark & E, \mathcodepanelextended & 18 & SCRIPT enc., splits line breaks \\
BPE SCRIPT-enc GPT-4o & BPE & S & B & \cmark & P, M & 19 & SCRIPT enc., GPT-4o regex \\
BPE GPT-2 (bal.) & BPE & G2 & B & \xmark & P & 20 &  \\
BPE GPT-4o (all-eq.) & BPE & G & Eq & \xmark & P & 21 &  \\
BPE Claude (all-eq.) & BPE & C & Eq & \xmark & P & 22 &  \\
BPE Punct (all-eq.) & BPE & P & Eq & \xmark & P & 23 &  \\
BPE GPT-4o NFC (all-eq.) & BPE & G & Eq & \cmark & P & 24 &  \\
BPE GPT-4o (all-eq., no-rep.) & BPE & G & Eq & \xmark & E & 21 & no repeat-sampling \\
BPE GPT-4o (bal., mf50) & BPE & G & B & \xmark & -- & -- & raised file cap, null control \\
BPE NFC clean (bal.) & BPE & Cl & B & \cmark & P, M & 25 &  \\
BPE NFC clean plus2 (bal.) & BPE & Cl & B & \cmark & E, \mathcodepanelextended & 25 & plus2 apostrophe \\
BPE NFC clean plus3 (bal.) & BPE & Cl & B & \cmark & E, \mathcodepanelextended & 25 & plus3 apostrophe \\
SuperBPE PA-BPE GPT-4o & SuperBPE & G & B & \cmark & E & 26 & PA-BPE base \\
SuperBPE PA-BPE GPT-4o t64k & SuperBPE & G & B & \cmark & E & 26 & PA-BPE base \\
SuperBPE clean C2 (bal.) & SuperBPE & Cl & B & \cmark & P, M & 27 & PA-BPE base, C2 \\
SuperBPE clean C3 (bal.) & SuperBPE & Cl & B & \cmark & E, \mathcodepanelextended & 27 & PA-BPE base, C3 \\
SuperBPE Punct t64k & SuperBPE & P & B & \xmark & E & 28 &  \\
PA-BPE NFC GPT-4o HW & PA-BPE & G & B & \cmark & E & 15 & hybrid window \\
PA-BPE NFC clean & PA-BPE & Cl & B & \cmark & P & 29 &  \\
Unigram GPT-4o tuned & Unigram & G & B & \xmark & E & 11 & tuned hyperparams \\
BPE GPT-4o (highres) & BPE & G & Hr & \xmark & P & 30 & 6 langs \\
BPE GPT-4o (highmid) & BPE & G & Hm & \xmark & P & 31 & 21 langs \\
BPE Whitespace (bal.) & BPE & W & B & \xmark & -- & -- & control \\
Unigram Whitespace tuned (bal.) & Unigram & W & B & \xmark & -- & -- & control, SentencePiece, tuned 


==> tables_camera_ready/tokenizer-roster-body.tex <==
% Body of tab:tokenizer-roster (NEW, not yet in tokeval_camera_ready.tex -- an \input{} line for this table needs to be added by hand). Regenerable: this script writes THIS file only. Generated by scripts/generate_tokenizer_roster_table.py. DO NOT EDIT BY HAND.
\begin{longtable}{@{}p{3.1cm}p{4.6cm}p{2.0cm}cp{1.3cm}p{2.6cm}@{}}
\caption{Comprehensive tokenizer roster: every trained tokenizer configuration appearing anywhere in this paper. \textbf{Membership} codes: P = primary std-1B panel member (implies the extended std-1B panel too), E = extended std-1B panel member not in the primary panel, M = primary 20B math+code panel member (implies the extended 20B panel too), Mx = extended 20B math+code panel member not in the primary 20B panel, R = off-the-shelf reference (never in any panel or aggregate statistic), \textrm{-} = not a member of any current panel. Both axes are shown together (e.g. P/M) when both apply. \textbf{1.27B run} states which training run backs each row's std-1B numbers: \emph{seed42 retrain}, for tokenizers originally trained before a later software-environment fix and re-trained afterward under seed 42 to remove that effect, or \emph{original}, for tokenizers trained only once, already under the fixed environment; or that no std-1B run exists. \textbf{20B} reports whether a 20B math+code checkpoint exists, independent of panel membership (e.g.\ the code-fraction-gradient rows have 20B checkpoints but are mechanism arms, not panel members). Collapsed rows (vocab ladder, code-fraction gradient) list every constituent slug's pattern in the Slug column and apply every other column value uniformly across the group; a companion machine-readable file in the project's supplementary materials lists each constituent slug individually.}
\label{tab:tokenizer-roster} \\
\toprule
\textbf{Display name} & \textbf{Slug} & \textbf{1.27B run} & \textbf{20B} & \textbf{Member.} & \textbf{Note} \\
\midrule
\endfirsthead
\multicolumn{6}{l}{\textit{(continued)}} \\
\toprule
\textbf{Display name} & \textbf{Slug} & \textbf{1.27B run} & \textbf{20B} & \textbf{Member.} & \textbf{Note} \\
\midrule
\endhead
\bottomrule
\endfoot
Mistral-Nemo & (off-the-shelf) & seed42 retrain & \cmark & R & off-the-shelf reference \\
LLaMA-3 & (off-the-shelf) & seed42 retrain & \cmark & R & off-the-shelf reference \\
\midrule
BPE GPT-4o (all-eq.) & \texttt{allmulti-equal-bpe} & original & \xmark & P & - \\
BPE NFC clean (bal.) & \texttt{bpe-nfc-clean-balanced} & original & \cmark & P/M & - \\
Vocab ladder (5 sizes) & \texttt{bpe-nfc-clean-balanced-v\{64,96,128,160,200\}k} & original & \xmark & - & vocab ladder \\
Vocab ladder, param-scaled (5 sizes) & \texttt{bpe-nfc-clean-balanced-v\{64,96,128,160,200\}k-paramscaled} & original & \xmark & - & vocab ladder \\
BPE NFC clean plus2 (bal.) & \texttt{bpe-nfc-plus2-balanced} & original & \cmark & E/Mx & - \\
BPE NFC clean plus3 (bal.) & \texttt{bpe-nfc-plus3-balanced} & original & \cmark & E/Mx & - \\
BPE Claude (all-eq.) & \texttt{claude-allmulti-equal-bpe} & original & \xmark & P & - \\
BPE Claude (bal.) & \texttt{claude-balanced-bpe} & seed42 retrain & \cmark & P/M & - \\
BPE Claude NFC & \texttt{claude-balanced-nfc-bpe} & seed42 retrain & \cmark & P/M & - \\
Unigram Claude & \texttt{claude-balanced-unigram} & seed42 retrain & \cmark & P/M & - \\
BPE Claude (eng.) & \texttt{claude-english-bpe} & seed42 retrain & \cmark & M & byte-drop defect (defect-flagged 20B run, E4) \\
\texttt{clauderev-balanced-bpe} & \texttt{clauderev-balanced-bpe} & original & \cmark & - & measurement-invalid (NFD normalizer) \\
BPE GPT-2 (balanced) & \texttt{gpt2-balanced-bpe} & original & \xmark & P & results in \cref{tab:pretok-alphabet-controls}, not \cref{tab:main-results} \\
BPE GPT-4o NFC (all-eq.) & \texttt{gpt4o-allmulti-equal-nfc-bpe} & original & \xmark & P & - \\
BPE GPT-4o (all-eq., no-rep.) & \texttt{gpt4o-allmulti-equal-norepeat-bpe} & original & \xmark & E & - \\
BPE GPT-4o (bal.) & \texttt{gpt4o-balanced-bpe} & seed42 retrain & \cmark & P/M & - \\
BPE GPT-4o (bal., mf50) & \texttt{gpt4o-balanced-maxfiles50-bpe} & original & \xmark & - & null control \\
BPE GPT-4o NFC & \texttt{gpt4o-balanced-nfc-bpe} & seed42 retrain & \cmark & P/M & - \\
Unigram GPT-4o & \texttt{gpt4o-balanced-unigram} & seed42 retrain & \cmark & P/M & - \\
Unigram GPT-4o tuned & \texttt{gpt4o-balanced-unigram-tuned} & original & \xmark & E & - \\
BPE GPT-4o (code) & \texttt{gpt4o-code-bpe} & seed42 retrain & \cmark & P/M & - \\
Code-fraction gradient (GPT-4o regex) & \texttt{gpt4o-codegrad\{00,05,30,50\}-bpe} & no std-1B run & \cmark & - & regex ablation (results in \cref{tab:axes2-grid}) \\
BPE GPT-4o (eng.) & \texttt{gpt4o-english-bpe} & seed42 retrain & \cmark & - & byte-drop defect \\
BPE GPT-4o (eng., full-byte) & \texttt{gpt4o-english-fullbyte-bpe} & original & \cmark & P/M & results in \cref{tab:pretok-alphabet-controls}, not \cref{tab:main-results} \\
GPT-4o NONL regex, balanced data (gradient anchor) & \texttt{gpt4onl-balanced-bpe} & no std-1B run & \cmark & - & regex ablation anchor (fusing counterpart: \texttt{gpt4o-balanced-bpe}); this tokenizer's own results are not printed in this paper \\
Code-fraction gradient (GPT-4o NONL regex) & \texttt{gpt4onl-codegrad\{00,05,30,50\}-bpe} & no std-1B run & \cmark & - & regex ablation (results in \cref{tab:axes2-grid}) \\
BPE GPT-4o (highmid) & \texttt{highmid-bpe} & original & \xmark & P & - \\
Unigram GPT-4o (highmid) & \texttt{highmid-unigram} & original & \xmark & P & - \\
BPE GPT-4o (highres) & \texttt{highres-bpe} & original & \xmark & P & - \\
Unigram GPT-4o (highres) & \texttt{highres-unigram} & original & \xmark & P & - \\
PA-BPE NFC clean & \texttt{pabpe-nfc-clean-balanced} & original & \xmark & P & - \\
PA-BPE NFC GPT-4o & \texttt{pabpe-nfc-gpt4-balanced} & original & \cmark & P/M & - \\
PA-BPE NFC GPT-4o HW & \texttt{pabpe-nfc-gpt4-balanced-hybridwindow} & original & \xmark & E & - \\
BPE Punct (all-eq.) & \texttt{punct-allmulti-equal-bpe} & original & \xmark & P & - \\
BPE Punct (bal.) & \texttt{punct-balanced-bpe} & seed42 retrain & \cmark & P/M & - \\
SuperBPE Punct t64k & \texttt{punct-balancedhalf-superbpe-t64k-copy} & original & \xmark & E & - \\
BPE Punct (eng.) & \texttt{punct-english-bpe} & seed42 retrain & \cmark & P/M & - \\
BPE RightAlign (bal.) & \texttt{rightalign-balanced-bpe} & seed42 retrain & \cmark & P/M & - \\
BPE RightAlign NFC & \texttt{rightalign-balanced-nfc-bpe} & seed42 retrain & \cmark & P/M & - \\
Unigram RightAlign & \texttt{rightalign-balanced-unigram} & seed42 retrain & \cmark & P/M & - \\
BPE SCRIPT-enc GPT-4o & \texttt{scripttok-bpe-scriptenc\_gpt4o\_cb} & original & \cmark & P/M & - \\
MinGram SCRIPT-enc & \texttt{scripttok-mingram-scriptenc\_cb} & original & \cmark & P/M & - \\
MinGram SCRIPT-enc (nl-split) & \texttt{scripttok-mingram-scriptenc\_cb\_nl} & original & \cmark & E/Mx & - \\
SuperBPE clean C2 (bal.) & \texttt{superbpe-clean-c2-balanced} & original & \cmark & P/M & - \\
SuperBPE clean C3 (bal.) & \texttt{superbpe-clean-c3-balanced} & original & \cmark & E/Mx & - \\
SuperBPE GPT-4o (bal.) & \texttt{superbpe-gpt4o-balanced} & original & \cmark & P/M & - \\
SuperBPE PA-BPE GPT-4o & \texttt{superbpe-pabpe-nfc-gpt4-balanced} & original & \xmark & E & - \\
SuperBPE PA-BPE GPT-4o t64k & \texttt{superbpe-pabpe-nfc-gpt4-t64k} & original & \xmark & E & - \\
BPE Whitespace (balanced) & \texttt{whitespace-balanced-bpe} & original & \cmark & - & failure probe \\
Unigram Whitespace tuned (balanced) & \texttt{whitespace-balanced-unigram} & original & \xmark & - & failure probe \\
\texttt{whitespace-multiheavy-bpe} & \texttt{whitespace-multiheavy-bpe} & original & \xmark & - & failure probe \\
\end{longtable}


==> tables_camera_ready/vocab-ladder-body.tex <==
% Body of tab:vocab-ladder in tokeval_camera_ready.tex. Regenerable: table scripts must write THIS file only; the caption lives in the main tex and is hand-maintained.
% Generated by scripts/generate_ablation_std1b_tables.py. DO NOT EDIT BY HAND.
\small
\begin{tabular}{llcccc}
\toprule
\textbf{Vocab} & \textbf{Condition} & \textbf{Val BPB} & \textbf{FLORES (tr.\ mean)} & \textbf{BLiMP} & \textbf{Code BPB} \\
\midrule
64k & byte-matched & $0.7193$ & $1.1630$ & $0.8131$ & $0.5269$ \\
64k & param-scaled & $0.7239$ & $1.1675$ & $0.8254$ & $0.5307$ \\
96k & byte-matched & $0.7186$ & $1.1645$ & $0.8217$ & $0.5264$ \\
96k & param-scaled & $0.7183$ & $1.1595$ & $0.8261$ & $0.5249$ \\
128k & byte-matched & $0.7162$ & $1.1585$ & $0.8208$ & $0.5244$ \\
128k & param-scaled & $0.7162$ & $1.1578$ & $0.8200$ & $0.5240$ \\
160k & byte-matched & $0.7143$ & $1.1569$ & $0.8269$ & $0.5210$ \\
160k & param-scaled & $0.7116$ & $1.1524$ & $0.8256$ & $0.5202$ \\
200k & byte-matched & $0.7128$ & $1.1584$ & $0.8153$ & $0.5193$ \\
200k & param-scaled & $0.7084$ & $1.1544$ & $0.8114$ & $0.5180$ \\
\bottomrule
\end{tabular}

